Towards Integrated Modelling of Dynamic Access Control with UML and Event-B

Role-Based Access Control (RBAC) is a popular authorization model used to manage data-access constraints in a wide range of systems. RBAC usually defines the static view on the access rights. However, to ensure dependability of a system, it is often necessary to model and verify state-dependent access rights. Such a modelling allows us to explicitly define the dependencies between the system states and permissions to access and modify certain data. In this paper, we present a work-in-progress on combining graphical and formal modelling to specify and verify dynamic access control. The approach is illustrated by a case study -- a reporting management system.

==> eptcsdata.tex <==
\providecommand{\firstpage}{105}
\providecommand{\publicationstatus}{R. Laleau, D. M\'ery, S. Nakajima, E. Troubitsyna (Eds): Joint Workshop on\\ Handling IMPlicit and EXplicit knowledge in formal system development\\ and  Formal \& Model-Driven Techniques for Developing Trustworthy Systems.\\
EPTCS 271, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.271.8}{10.4204/EPTCS.271.8}}
\pdfoutput=1

